Optimal Multi-Robot Communication-Aware Trajectory Planning by Constraining the Fiedler Value

The paper present a novel approach for the solution of the Multi-Robot Communication-Aware Trajectory Planning, which builds on a general optimisation framework where the changes in robots positions are used as decision variable, and linear constraints on the trajectories of the robots are introduced to ensure communication performance and collision avoidance. The Fiedler value is adopted as communication performance metric. The validity of the method in computing both feasible and optimal trajectories for the robots is demonstrated both in simulation and experimentally. Results show that the constraint on the Fiedler value ensures that the robot network fulfils its objective while maintaining communication connectivity at all times. Further, the paper shows that the introduction of approximations for the constraints enables a significant improvement in the computational time of the solution, which remain very close to the optimal solution.

==> sections/algorithm.tex <==
\section{Algorithm}

==> sections/experiment.tex <==
\section{Experiment Results}
To verify the deployability of the MR-CaTP algorithm, it is implemented on the MRS UAV System \cite{Baca2020TheVehicles}. The MRS UAV system does not use ad-hoc communication but instead relies on infrastructure based communication. Therefore the experimental results cannot be used to analyse the effect of the planner on the communication performance, but have only been used to validate that the planner produces trajectories that are feasible for the UAVs to track.
\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{figs/swarm_picture.png}
    \caption{MRS UAV swarm. Red circles highlight the positions of the UAVs.}
    \label{fig:swarm_picture}
\end{figure}
To test the algorithm $N=6$ UAVs were deployed to inspect $L=3$ POIs. Four experiments were conducted with the same POI positions and varying initial position of the UAVs. As can be seen in \cref{fig:exp1}, \ref{fig:exp2}, \ref{fig:exp3}, and \ref{fig:exp4}, the terminal positions of the UAVs are highly dependent on their initial positions. In \cref{fig:exp1} and \ref{fig:exp4} two of the UAVs terminate in positions that are clearly sub-optimal. They are moved there to support the movement of the inspection UAVs and are stuck there, either due to not being able to circumnavigate the inspection UAV or due to the cost of movement being too steep. In \cref{fig:exp3} an example of a clearly optimal configuration can be seen, where the robots that are not assigned to POIs are positioned inside the convex hull of the POI. In \cref{fig:exp1}, \ref{fig:exp2}, \ref{fig:exp3}, and \ref{fig:exp4}, the green lines indicate communication links where the PRR is greater than $5\%$. As can be seen, the terminal positions of the UAVs generate configurations where the network remains connected. In \cref{fig:exp1}, \ref{fig:exp2}, \ref{fig:exp3}, and \ref{fig:exp4}, the Fiedler value can also be seen along with the desired lower bound and the Fiedler value if the unassigned UAVs remained stationary. It is clear to see that the MR-CaTP algorithm keeps the Fiedler value above the lower bound, and that the Fiedler value would fall below the lower bound if the MR-CaTP algorithm were not used. Lastly, in \cref{fig:exp1} and \ref{fig:exp2} it can be seen that the Fiedler value reaches the lower bound, and that the communication constraint in the MR-CaTP algorithm therefore successfully ensures that communication is preserved.  
\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{figs/exp1.eps}
    \caption{MR-CaTP experiment number 1.}
    \label{fig:exp1}
\end{figure}
\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{figs/exp2.eps}
    \caption{MR-CaTP experiment number 2.}
    \label{fig:exp2}
\end{figure}
\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{figs/exp3.eps}
    \caption{MR-CaTP experiment number 3.}
    \label{fig:exp3}
\end{figure}
\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{figs/exp4.eps}
    \caption{MR-CaTP experiment number 4.}
    \label{fig:exp4}
\end{figure}
